Search for 100 MeV to 10 GeV gamma-ray lines in the Fermi-LAT data and implications for gravitino dark matter in the $\mu\nu$SSM

Dark matter decay or annihilation may produce monochromatic signals in the gamma-ray energy range. In this work we argue that there are strong theoretical motivations for studying these signals in the framework of gravitino dark matter decay and we perform a search for gamma-ray spectral lines from 100\,MeV to 10\,GeV with Fermi-LAT data. In contrast to previous line searches at higher energies, the sensitivity of the present search is dominated by systematic uncertainties across most of the energy range considered. We estimate the size of systematic effects by analysing the flux from a number of control regions, and include the systematic uncertainties consistently in our fitting procedure. We have not observed any significant signals and present model-independent limits on gamma-ray line emission from decaying and annihilating dark matter. We apply the former limits to the case of the gravitino, a well-known dark matter candidate in supersymmetric scenarios. In particular, the $R$-parity violating "$\mu$ from $\nu$" Supersymmetric Standard Model ($\mu\nu$SSM) is an attractive scenario in which including right-handed neutrinos solves the $\mu$ problem of the Minimal Supersymmetric Standard Model while simultaneously explaining the origin of neutrino masses. At the same time, the violation of $R$-parity renders the gravitino unstable and subject to decay into a photon and a neutrino. As a consequence of the limits on line emission, $\mu\nu$SSM gravitinos with masses larger than about 5\,GeV, or lifetimes smaller than about $10^{28}$\,s, are excluded at 95% confidence level as dark matter candidates.

==> README <==
The top level tex file is LowEnergyLines.tex.  This file has the abstract
and acknowledgments in it.  All other pieces (sections, appendicies, etc) should
be included as separate .tex files (i.e. intro.tex)

Refer to fermiStyle.tex for commonly used LAT phrases and their formatting.  For
example, please use "\stools" instead of typing "Science Tools" as there is LAT
collaboration formatting that we like to use for that phrase.

Refer to thisPaperStyle.tex for common variable names and formatting.  For
example, use "\Ereco" when referring to the reconstructed energy of an event to
get the correct formatting.  Please add any common variables you think are
missing from this list for the Low Energy Line analysis.  

thisPaperStyle also contains functions for lists (\fermienumerate and
\fermiitemize) and plotting (\twopanel)
Here is an example of how to use the plotting functions:
\onepanel{}{RelicDensity7}{\caption{Gravitino mass--reheating temperature plane. The thick lines show the contours where the gravitino relic density matches the observed dark matter density for a given value of the gluino mass according to Eq.~\eqref{gravitinorelic1}. We show the case of universal gaugino masses at the GUT scale. Low values of the gluino mass are excluded by collider searches while large values are disfavoured by the hierarchy problem. In the upper right corner (green region) the gravitino is lighter than the Bino and thus cannot be a DM candidate. In the particular case of the $\mu\nu$SSM, gravitino masses above roughly 4\,GeV (orange region) are excluded by gamma-ray line searches (see Section~\ref{results}). See text for details.
}\label{fig:relicdensity}}

For ALL figures:
1)  Please create a macro (put in macros/) that plots something (put numbers/tables in
macros/data/...only small files like .txt files or root files with a few
histograms, we don't need to clog the area with large data files like the whole
sky ROOT tree)
2) macros should use pyRoot and import RootStyles to ensure we have common
plotting styles.  See macros/example_FracVsEn.py for an example
3) Please put a .eps and .pdf version of the plot in figs/  Like the HE paper, we can keep png versions in
figs/png.  If you use the can.save() function from RootStyle.py, you will automatically create all three types
of plots (eps, pdf, png).  See macros/example_FracVsEn.py

To compile the paper (as a PDF) do
"make clean"
"make pdf"

Please don't commit any conflicts!  check with "svn status"

